TEAM: a parameter-free algorithm to teach collaborative robots motions from user demonstrations

Learning from demonstrations (LfD) enables humans to easily teach collaborative robots (cobots) new motions that can be generalized to new task configurations without retraining. However, state-of-the-art LfD methods require manually tuning intrinsic parameters and have rarely been used in industrial contexts without experts. We propose a parameter-free LfD method based on probabilistic movement primitives, where parameters are determined using Jensen-Shannon divergence and Bayesian optimization, and users do not have to perform manual parameter tuning. The cobot's precision in reproducing learned motions, and its ease of teaching and use by non-expert users are evaluated in two field tests. In the first field test, the cobot works on elevator door maintenance. In the second test, three factory workers teach the cobot tasks useful for their daily workflow. Errors between the cobot and target joint angles are insignificant -- at worst 0.28 deg -- and the motion is accurately reproduced -- GMCC score of 1. Questionnaires completed by the workers highlighted the method's ease of use and the accuracy of the reproduced motion. Public implementation of our method and datasets are made available online.

==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

\def\gnuplot@output@ps{ps} % required for comparison in \gprawimage

\expandafter\def\csname gnuplot@select@driver@pgfsys-dvi.def\endcsname     {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfm.def\endcsname {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvipdfmx.def\endcsname{pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-dvips.def\endcsname   {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-pdftex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-luatex.def\endcsname  {pdf}
\expandafter\def\csname gnuplot@select@driver@pgfsys-tex4ht.def\endcsname  {html}
\expandafter\def\csname gnuplot@select@driver@pgfsys-textures.def\endcsname{ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-vtex.def\endcsname    {ps}
\expandafter\def\csname gnuplot@select@driver@pgfsys-xetex.def\endcsname   {pdf}

\ifcsname gnuplot@select@driver@\pgfsysdriver\endcsname
  \edef\gnuplot@output@mode{\csname gnuplot@select@driver@\pgfsysdriver\endcsname}
\else
  \errmessage{The driver \pgfsysdriver\space is not supported by gnuplot-lua-tikz}%
\fi

\ifcsname PackageWarning\endcsname
  \let\gnuplot@packagewarning\PackageWarning
\else
  \def\gnuplot@packagewarning#1#2{\immediate\write-1{Package #1 Warning: #2}}
\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
  \gnuplot@packagewarning{gnuplot-lua-tikz}{%
    \noexpand\gp@rawimage is not implemented for \gnuplot@output@mode\space output.%
  }%
}

% Select \gp@rawimage depending on the output mode
\expandafter\let\expandafter\gp@rawimage\csname gp@rawimage@\gnuplot@output@mode\endcsname

\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{%
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext{%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
  \else
    \ifx\gnuplot@output@mode\gnuplot@output@ps
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}%
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}%
    \fi
  \fi
}

%
% gnuplottex compatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
% 3-parameter variant gp3point passes style options as well as point type and coordinates
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}
\def\gp3point#1#2#3{%
  \path[solid#2] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#3};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}%
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }%
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex,line width=0pt}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex,line width=0pt}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex,line width=0pt}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
%%
%%  plain TeX wrapper for gnuplot-tikz style file
%%
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds,fit}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode

\endinput


==> images/bayesian_stability.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.4p3 (Lua 5.4; terminal rev. Jun 2020, script rev. 115)
%% Tue 30 May 2023 11:14:12 PM CEST
\tikzset{every node/.append style={font={\footnotesize}}}
\gpcolor{rgb color={0.502,0.502,0.502}}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{1.00}
\draw[gp path] (1.320,0.924)--(8.447,0.924);
\gpcolor{rgb color={0.000,0.620,0.451}}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\draw[gp path] (1.320,0.924)--(1.500,0.924);
\node[gp node right] at (1.136,0.924) {$0$};
\gpcolor{rgb color={0.502,0.502,0.502}}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\draw[gp path] (1.320,1.477)--(8.447,1.477);
\gpcolor{rgb color={0.000,0.620,0.451}}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\draw[gp path] (1.320,1.477)--(1.500,1.477);
\node[gp node right] at (1.136,1.477) {$20$};
\gpcolor{rgb color={0.502,0.502,0.502}}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\draw[gp path] (1.320,2.031)--(8.447,2.031);
\gpcolor{rgb color={0.000,0.620,0.451}}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\draw[gp path] (1.320,2.031)--(1.500,2.031);
\node[gp node right] at (1.136,2.031) {$40$};
\gpcolor{rgb color={0.502,0.502,0.502}}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\draw[gp path] (1.320,2.584)--(8.447,2.584);
\gpcolor{rgb color={0.000,0.620,0.451}}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\draw[gp path] (1.320,2.584)--(1.500,2.584);
\node[gp node right] at (1.136,2.584) {$60$};
\gpcolor{rgb color={0.502,0.502,0.502}}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\draw[gp path] (1.320,3.138)--(8.447,3.138);
\gpcolor{rgb color={0.000,0.620,0.451}}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\draw[gp path] (1.320,3.138)--(1.500,3.138);
\node[gp node right] at (1.136,3.138) {$80$};
\gpcolor{rgb color={0.502,0.502,0.502}}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\draw[gp path] (1.320,3.691)--(8.447,3.691);
\gpcolor{rgb color={0.000,0.620,0.451}}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\draw[gp path] (1.320,3.691)--(1.500,3.691);
\node[gp node right] at (1.136,3.691) {$100$};
\draw[gp path] (1.320,3.691)--(1.320,0.924)--(8.447,0.924);
\gpcolor{color=gp lt color border}
\node[gp node center,rotate=-270] at (0.292,2.307) {Time (s)};
\node[gp node left] at (0.753,0.334) {T1};
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (1.305,0.257)--(2.221,0.257)--(2.221,0.411)--(1.305,0.411)--cycle;
\draw[gp path] (8.192,1.375)--(8.320,1.375)--(8.320,1.516)--(8.192,1.516)--cycle;
\draw[gp path] (8.192,1.471)--(8.320,1.471);
\draw[gp path] (8.256,1.265)--(8.256,1.375);
\draw[gp path] (8.256,1.516)--(8.256,1.668);
\draw[gp path] (8.220,1.668)--(8.292,1.668);
\draw[gp path] (8.220,1.265)--(8.292,1.265);
\gpcolor{color=gp lt color border}
\node[gp node left] at (2.405,0.334) {T2};
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (2.957,0.257)--(3.873,0.257)--(3.873,0.411)--(2.957,0.411)--cycle;
\draw[gp path] (3.154,1.511)--(3.282,1.511)--(3.282,1.705)--(3.154,1.705)--cycle;
\draw[gp path] (3.154,1.627)--(3.282,1.627);
\draw[gp path] (3.218,1.271)--(3.218,1.511);
\draw[gp path] (3.218,1.705)--(3.218,1.945);
\draw[gp path] (3.182,1.945)--(3.254,1.945);
\draw[gp path] (3.182,1.271)--(3.254,1.271);
\gpsetpointsize{4.00}
\gp3point{gp mark 7}{}{(3.218,2.127)}
\gp3point{gp mark 7}{}{(3.218,2.336)}
\gp3point{gp mark 7}{}{(3.218,2.365)}
\gp3point{gp mark 7}{}{(3.218,2.997)}
\gpcolor{color=gp lt color border}
\node[gp node left] at (4.057,0.334) {T3};
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (4.609,0.257)--(5.525,0.257)--(5.525,0.411)--(4.609,0.411)--cycle;
\draw[gp path] (4.978,1.212)--(5.106,1.212)--(5.106,1.308)--(4.978,1.308)--cycle;
\draw[gp path] (4.978,1.278)--(5.106,1.278);
\draw[gp path] (5.042,1.148)--(5.042,1.212);
\draw[gp path] (5.042,1.308)--(5.042,1.396);
\draw[gp path] (5.006,1.396)--(5.078,1.396);
\draw[gp path] (5.006,1.148)--(5.078,1.148);
\gpcolor{color=gp lt color border}
\node[gp node left] at (5.709,0.334) {T4};
\gpcolor{rgb color={0.902,0.624,0.000}}
\draw[gp path] (6.261,0.257)--(7.177,0.257)--(7.177,0.411)--(6.261,0.411)--cycle;
\draw[gp path] (1.448,1.378)--(1.576,1.378)--(1.576,1.703)--(1.448,1.703)--cycle;
\draw[gp path] (1.448,1.442)--(1.576,1.442);
\draw[gp path] (1.512,1.146)--(1.512,1.378);
\draw[gp path] (1.512,1.703)--(1.512,2.146);
\draw[gp path] (1.476,2.146)--(1.548,2.146);
\draw[gp path] (1.476,1.146)--(1.548,1.146);
\gp3point{gp mark 7}{}{(1.511,2.261)}
\gp3point{gp mark 7}{}{(1.511,2.351)}
\gp3point{gp mark 7}{}{(1.511,2.559)}
\gp3point{gp mark 7}{}{(1.511,2.685)}
\gp3point{gp mark 7}{}{(1.511,2.700)}
\gp3point{gp mark 7}{}{(1.511,3.100)}
\gp3point{gp mark 7}{}{(1.511,3.589)}
\gpcolor{color=gp lt color border}
\node[gp node left] at (7.361,0.334) {T5};
\gpcolor{rgb color={0.941,0.894,0.259}}
\draw[gp path] (7.913,0.257)--(8.829,0.257)--(8.829,0.411)--(7.913,0.411)--cycle;
\draw[gp path] (3.044,1.233)--(3.172,1.233)--(3.172,1.310)--(3.044,1.310)--cycle;
\draw[gp path] (3.044,1.270)--(3.172,1.270);
\draw[gp path] (3.108,1.169)--(3.108,1.233);
\draw[gp path] (3.108,1.310)--(3.108,1.405);
\draw[gp path] (3.072,1.405)--(3.144,1.405);
\draw[gp path] (3.072,1.169)--(3.144,1.169);
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (1.320,3.691)--(1.320,0.924)--(8.447,0.924);
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.320cm}{0.924cm}}{\pgfpoint{8.447cm}{3.691cm}}
\end{tikzpicture}
%% gnuplot variables


==> limitations.tex <==
\section{Limitations and future work}

TEACH cannot handle sets including widely different demonstrations.
While DTW is enough to use demonstration with different time lengths, TEACH estimate the motion of the cobot based on joint angles, thus the same motion from two different cobot poses will lead to an incorrect motion model---see \cref{fig:limitations:trajectory}.
This drawback can be overcome by preprocessing the demonstration before training to be in similar reference frame.
We leave this for future work.

For now, the full training procedure of TEACH must be run every time a new demonstration is added.
This training time is the longest part when using the cobot.
To reduce the training time, in future work, we will work on updating the model parameters incrementally.

As shown by \textcite{Ijspeert2013Nonlinear}, the damped spring model can handle obstacles in the environment.
In future work, we plan to add the ability for TEACH to handle obstacles using external sensors such as a 3D camera.

==> results/results_table.tex <==

\begin{table*}[!ht]
    \centering
    \scalebox{0.7}{\begin{tabular}{l  c  c  c  c  c  c  c  c  c}
            \toprule
            Task                                         & T1                 & T2                & T3                & T4                & T5                & F1                              & F2                & F3               & F4                \\ [0.5ex]
            \midrule
            \makecell[l]{Name}                           & \makecell{Open the                                                                                                                                                                              \\ door} & \makecell{Pick up\\ brush} & \makecell{Clean\\ rail} & \makecell{Deposit\\ brush} & \makecell{Close the\\ door} & \makecell{Drill} & \makecell{Avoid} & \makecell{Parallel} & \makecell{Collaborative}\\
            \addlinespace[0.5em]
            \makecell[l]{Nb demonstrations}              & 6                  & 4                 & 4                 & 4                 & 3                 & 3                               & 3                 & 3                & 3                 \\
            \addlinespace[0.5em]
            \makecell[l]{Average demonstration                                                                                                                                                                                                             \\ duration [s]} & $33.188\pm2.383$ & $36.37\pm2.277$ & $32.926\pm3.000$ & $28.167\pm3.326$ &  $26.187\pm1.047$ & $22.601\pm5.876$ & $33.41\pm6.483$ & $23.301\pm3.528$ & $22.121\pm3.445$\\
            \addlinespace[0.5em]
            \makecell[l]{DTW [s]}                        & $104.411\pm0.637$  & $104.346\pm1.607$ & $93.268\pm0.529$  & $67.751\pm2.918$  & $56.574\pm1.572$  & $16.299\pm0.884$                & $38.779\pm0.372$  & $27.327\pm0.443$ & $12.727\pm0.236$  \\
            \addlinespace[0.5em]
            \makecell[l]{GMM + GMR [s]}                  & $64.538\pm1.156$   & $77.817\pm3.287$  & $79.679\pm0.528$  & $75.273\pm2.861$  & $78.113\pm2.388$  & $60.886\pm3.813$                & $65.526\pm0.931$  & $53.151\pm0.756$ & $64.56\pm0.978$   \\
            \addlinespace[0.5em]
            \makecell[l]{BO [s]}                         & $14.693\pm1.568$   & $20.783\pm1.915$  & $12.464\pm2.824$  & $19.555\pm2.211$  & $13.547\pm2.532$  & $20.983\pm17.845$               & $11.934\pm1.767$  & $11.027\pm3.540$ & $14.649\pm14.418$ \\
            \addlinespace[0.5em]
            \makecell[l]{ProMP[s]}                       & $0.442\pm0.009$    & $0.387\pm0.014$   & $0.409\pm0.007$   & $0.310\pm0.016$   & $0.352\pm0.040$   & $0.261\pm0.035$                 & $0.464\pm0.016$   & $0.327\pm0.016$  & $0.277\pm0.046$   \\
            \addlinespace[0.5em]
            \makecell[l]{Total time [s]}                 & $184.084\pm2.452$  & $203.334\pm4.316$ & $185.819\pm3.074$ & $162.888\pm4.558$ & $148.586\pm4.506$ & $98.428\pm18.924$               & $116.704\pm2.176$ & $91.832\pm3.505$ & $92.213\pm14.639$ \\
            \addlinespace[0.5em]
            \makecell[l]{Position error $e_p$ [mm]}      & $1.058\pm0.278$    & $0.895\pm0.005$   & $1.479\pm0.351$   & $0\pm0$           & $0.726\pm0.011$   & $0\pm0$                         & $0.153\pm0.026$   & $0.536\pm0.646$  & $0.295\pm0.291$   \\
            \addlinespace[0.5em]
            \makecell[l]{Orientation error $e_{\theta}$} & $0.002\pm0.001$    & $0.004\pm0.001$   & $0.005\pm0.002$   & $0.001\pm10^{-5}$ & $0.002\pm10^{-5}$ & \makecell[c]{$5.2\cdot10^{-5} $                                                            \\ $\pm3.4\cdot10^{-5}$} & \makecell[c]{$9.6\cdot10^{-4}$\\$ \pm7.2\cdot 10^{-4}$} & \makecell[c]{$4.7\cdot10^{-4}$\\$\pm5.5\cdot10^{-4}$} & $0.001\pm0.001$   \\
            \addlinespace[0.5em]
            \makecell[l]{Joints error $e_{j}$ [rad]}     & $0.013\pm0.006$    & $0.008\pm0.003$   & $0.007\pm0.002$   & $0.008\pm0.002$   & $0.007\pm0.002$   & $0.618\pm0.517$                 & $0.580\pm0.274$   & $0.573\pm0.228$  & $0.594\pm0.199$   \\
            \addlinespace[0.5em]
            \makecell[l]{Failures}                       & 0                  & 0                 & 0                 & 0                 & 0                 & 0                               & 0                 & 0                & 0                 \\
            \bottomrule
        \end{tabular}}
    \caption{
        This table presents for each task: the number of collected demonstrations per task, the average duration of a demonstration in the dataset, the time taken by each step of \projectName{} during trainings, and the results for each error metric---respectively 10 and 30 runs are performed for the door maintenance and the factory tasks.
        Failures correspond to the number of time the robot either by not reproducing the movement or failed at completing the task---this was evaluated visually.
        \vspace{-8mm}
    }
    \label{data-sets}
\end{table*}

==> results/table_maintenance.tex <==

\begin{table*}[!ht]
    \centering
    \begin{tabular}{l  c  c  c  c  c}
        \toprule
        Task                                             & T1                 & T2                 & T3                & T4                & T5                \\ [0.5ex]
        \midrule
        % \makecell[l]{Name}                               & \makecell{Open the                                                                                  \\ door} & \makecell{Pick up \\brush} & \makecell{Clean \\ rail} & \makecell{Deposit \\ brush} & \makecell{Close the \\ door} \\
        \addlinespace[0.5em]
        \makecell[l]{Nb demonstrations}                  & 6                  & 4                  & 4                 & 4                 & 3                 \\
        \addlinespace[0.5em]
        \makecell[l]{Average demonstration duration [s]} & 33.196$\pm$2.384   & 36.373$\pm$2.285   & 32.932$\pm$3.001  & 28.161$\pm$3.332  & 26.192$\pm$1.057  \\
        \addlinespace[0.5em]
        \makecell[l]{DTW [s]}                            & 116.615$\pm$7.819  & 113.703$\pm$4.646  & 100.385$\pm$3.517 & 69.537$\pm$1.566  & 58.943$\pm$3.861  \\
        \addlinespace[0.5em]
        \makecell[l]{GMM + GMR [s]}                      & 72.005$\pm$5.264   & 92.404$\pm$7.153   & 87.104$\pm$2.553  & 80.613$\pm$4.282  & 82.972$\pm$5.821  \\
        \addlinespace[0.5em]
        \makecell[l]{ProMP [s]}                          & 25.158$\pm$3.840   & 23.645$\pm$2.046   & 22.840$\pm$0.624  & 17.912$\pm$0.747  & 18.742$\pm$1.601  \\
        \addlinespace[0.5em]
        \makecell[l]{Total time [s]}                     & 213.775$\pm$13.702 & 229.740$\pm$10.573 & 210.328$\pm$4.908 & 168.055$\pm$5.571 & 160.667$\pm$8.928 \\
        \addlinespace[0.5em]
        \makecell[l]{Position error $e_p$ [mm]}          & 1.058$\pm$0.278    & 0.895$\pm$0.005    & $1.479\pm0.351$   & 0 $\pm$ 0         & 0.726$\pm$0.011   \\
        \addlinespace[0.5em]
        \makecell[l]{Orientation error $e_{\theta}$}     & 0.002$\pm$0.001    & 0.004$\pm$0.001    & 0.005$\pm$0.002   & 0.001$\pm10^{-5}$ & 0.002$\pm10^{-5}$ \\
        \addlinespace[0.5em]
        \makecell[l]{Joints error $e_{j}$ [rad]}         & 0.013$\pm$0.006    & 0.008$\pm$0.003    & 0.007$\pm$0.002   & 0.008$\pm$0.002   & 0.007$\pm$0.002   \\
        \addlinespace[0.5em]
        \makecell[l]{Failures}                           & 0                  & 0                  & 0                 & 0                 & 0                 \\
        \bottomrule
    \end{tabular}
    \caption{
        This table presents for each task: the number of collected demonstrations per task, the average duration of a demonstration in the dataset.
        Furthermore, the time taken by each step of \projectName{} for 10 trainings, and the error metrics for 10 reproductions are presented.
        Failures is the number of time the robot either by not reproducing the movement or failed at completing the task---this was evaluated visually by the user.
        % Since, T1 and T2 have the largest datasets---in number and length of demonstrations---those tasks have the longest training time.
        % On the other hand, T4 and T5, have the shortest training time.
    }
    \label{data-sets-lab}
\end{table*}





% \begin{table}[t]
%     \centering
%      \scalebox{0.8}{\begin{tabular}{l  c  c  c  c  c}
%      \toprule
%       Task & T1 & T2 & T3 & T4 & T5 \\ [0.5ex]
%      \midrule
%     \makecell[l]{Position error $e_p$ [mm]}  & 1.058$\pm$0.278 & 0.895$\pm$0.005 & 1.479$\pm$0.351 & 0 & 0.726$\pm$0.011 \\
%     \addlinespace[0.5em]
%      \makecell[l]{Orientation error $e_{\theta}$} & 0.002$\pm$0.001 & 0.004$\pm$0.001 & 0.005$\pm$0.002 & 0.001$\pm10^{-5}$ & 0.002$\pm10^{-5}$\\
%      \addlinespace[0.5em]
%      \makecell[l]{Joints error $e_{j}$ [rad]} & 0.013$\pm$0.006 & 0.008$\pm$0.003 & 0.007$\pm$0.002 & 0.008$\pm$0.002 & 0.007$\pm$0.002\\
%      \bottomrule
%     \end{tabular}}
%     \caption{This table presents the position, orientation and joints error of the endpoint robot trajectory with respect to the task target. T1 and T3 are the tasks with the largest position errors. Those tasks require interaction between the tool and the object. Notably, contact interaction between the brush sponge and the rail surface, and magnetic interaction between the tool magnets and the metal plate. This interaction adds a challenge for the user to understand which is the correct release point, due to sponge deformation or magnetic attraction. T2 and T3 are the tasks with the largest orientation error. This is again caused by the sponge deformation at the contact point that prevents the user to clearly understand the final tool configuration. The joints error is similar for all tasks and it is slightly higher for T1 since it is the task with the largest robot joint displacements along the trajectory.}
%     \label{endpoint-accuracy}
%     \end{table}
